Heavy-tailed Streaming Statistical Estimation

We consider the task of heavy-tailed statistical estimation given streaming $p$-dimensional samples. This could also be viewed as stochastic optimization under heavy-tailed distributions, with an additional $O(p)$ space complexity constraint. We design a clipped stochastic gradient descent algorithm and provide an improved analysis, under a more nuanced condition on the noise of the stochastic gradients, which we show is critical when analyzing stochastic optimization problems arising from general statistical estimation problems. Our results guarantee convergence not just in expectation but with exponential concentration, and moreover does so using $O(1)$ batch size. We provide consequences of our results for mean estimation and linear regression. Finally, we provide empirical corroboration of our results and algorithms via synthetic experiments for mean estimation and linear regression.

==> temp.tex <==

\begin{figure*}[h]
\vspace{-0.4cm}       
\centering
      \subfigure[\label{fig:linear_regression_convergence} \small{Expected convergence curve. }]{\includegraphics[width=0.28\textwidth]{figs/linear_regression/gamma_convergence.png} } \vspace{-0.12cm}\hfill
      \subfigure[\label{fig:linear_regression_quantile} \small{Last iteration quantile loss. }]{\includegraphics[width=0.28\textwidth]{figs/linear_regression/log_quantile.png}}
      \vspace{-0.12cm}\hfill
      \subfigure[\label{fig:linear_regression_lambda_vs_quantiles}\small{$\log_2(Q_\delta(\theta^N))$ v.s. $\lambda$.}]{\includegraphics[width=0.28\textwidth]{figs/linear_regression/lambda_vs_quantile.png}}
      \vspace{-0.12cm}
      
      \subfigure[\label{fig:linear_regression_gamma_vs_quantiles}\small{Expected convergence curve for different $\gamma$. }]{\includegraphics[width=0.28\textwidth]{figs/linear_regression/convergence_vs_gamma.png} }\hfill
      \subfigure[\label{fig:linear_regression_sigma_vs_quantiles}\small{$\log_2(Q_\delta(\theta^N))$ v.s. $\sigma^2$ for $\delta = 0.01$. }]{\includegraphics[width=0.28\textwidth]{figs/linear_regression/delta0.01_sigma^2_vs_quantile.png}} \hfill
      \subfigure[\label{fig:linear_regression_p_vs_quantiles}\small{$\log_2(Q_\delta(\theta^N))$ v.s. $p$ for $\delta = 0.01$ and $N = 1024$.}]{\includegraphics[width=0.28\textwidth]{figs/linear_regression/delta0.01_log_2(p)_vs_quantile.png}}
\vspace{-0.2cm}    
\caption{Results for robust linear regression for $N=1024, p = 256$, $\gamma=256$ and $\sigma^2 = 0.75$.}
\label{fig:linear_regression}
\vspace{-0.3cm}       
\end{figure*}



\section{Sketch of Proof}
\label{sec:sketch_of_proof}

In this section, we provide an overview of the arguments that constitute the proof of Theorem \ref{thm:clipped_sgd} and explain our theoretical contribution. The full details of the proof can be found in Appendix~\ref{sec:proof_clipped_sgd}. Our proof is improved upon previous analysis of clipped-SGD with constant learning rate and $O(n)$ batch size ~\citep{gorbunov2020stochastic} and high probability bounds for SGD with $O(1/t)$ step size in the sub-Gaussian setting~\citep{harvey2019simple}. Our analysis consists of three steps: (i) Expansion of the update rule. 
(ii) Selection of the clipping level. 
(iii) Concentration of bounded martingale sequences.

\paragraph{Notations:} Recall that we use step size $\eta_t = \frac{1}{\tau_\ell(t+\gamma)}$. We will write $\epsilon_t = \nabla \calR(\theta^{t}) - \clip(\nabla \loss(\theta^{t},\z_t), \lambda) $ is the noise indicating the difference between the stochastic gradient and the true gradient at step $t$. Let $\calF_t = \sigma(\z_1,\cdots,\z_t)$ be the $\sigma$-algebra generated by the first $t$ steps of \texttt{clipped-SGD}. We note that clipping introduce bias so that $\Exp_{\z_t}[\epsilon_t | \calF_{t-1}]$ is no longer zero, so we decompose the noise term $\epsilon_t = \epsilon_{t}^b + \epsilon_{t}^v$ into a bias term $\epsilon_{t}^b $ and a zero-mean variance term  $\epsilon_{t}^v $, i.e. 
$$\epsilon_t = \epsilon_{t}^b + \epsilon_{t}^v, 
\text{ where } 
\epsilon_{t}^b  = \Exp_{\z_t}[\epsilon_t| \calF_{t-1}]
\text{ and }
\epsilon_{t}^v  = \epsilon_t - \Exp_{\z_t}[\epsilon_t| \calF_{t-1}]
$$

\paragraph{(i) Expansion of the update rule:}  We start with the following lemma that is pretty standard in the analysis of SGD for strongly convex functions. It can be obtained by unrolling the update rules $\theta^{t+1} = \calP_\Theta \left(\theta^t - \eta_t \clip(\nabla \loss(\theta^t, \z_t),\lambda) \right)$ and using properties of $\tau_\ell$-strongly-convex and $\tau_u$-smooth functions.
\begin{lemma}
\label{lm:strongly_convex_expansion_main_paper}
Under the conditions in Theorem \ref{thm:clipped_sgd}, for any $1 \leq i \leq N$, we have
\begin{align*}
\small
\norm{\theta^{i+1} - \theta^*}{2}^2 
\leq  
\underbrace{\frac{\gamma(\gamma-1)\norm{\theta^1 - \theta^*}{2}^2 }{(i+\gamma)(i+\gamma-1)}}_{\text{the initialization error}} 
+ \underbrace{\frac{\sum_{t=1}^{i}  (t+\gamma-1) \inprod{\epsilon_t^b +\epsilon_t^v  }{\theta^t - \theta^*} }{\tau_\ell(i+\gamma)(i+\gamma-1)}}_{\text{the first noise term }} 
+ \underbrace{\frac{2\sum_{t=1}^{i} \left( \norm{ \epsilon_t^v }{2}^2 + \norm{ \epsilon_t^b }{2}^2 \right)} {\tau_\ell^2(i+\gamma)(i+\gamma-1)}}_{\text{the second noise term
}}. 
\end{align*}
\end{lemma}

\paragraph{(ii) Selection of the clipping level:} Now, to upper bound \textit{the noise terms}, 
we need to choose the clipping level $\lambda$ properly to balance the variance term $\epsilon_t^v$ and the bias term $\epsilon_t^b$. Specifically, we use the inequalities of \citet{gorbunov2020stochastic}, which provides us upper bounds for the magnitude and variance of these noise terms.
\begin{lemma}
\vspace{-0.1cm}
(Lemma F.5, \citep{gorbunov2020stochastic} )
For any $t=1,2,..,N$, we have
\begin{equation}
\norm{\epsilon_t^v}{2}
\leq  2\lambda.
\end{equation}
Moreover, for all $t=1,2,..,N$, assume that the variance of stochastic gradients is bounded by $\sigma_t^2$, i.e. $\Exp_{\z_t}[\norm{\nabla \loss(\theta^t, \z_t) - \nabla \calR(\theta^t)}{2}^2 | \calF_{t-1}] \leq \sigma_t^2 $ and assume that the norm of the true gradient is less than $\lambda/2$, i.e.
$ \norm{\nabla \calR(\theta^t)}{2} \leq \lambda/2$. Then we have
\begin{equation}
\label{eqn:b_and_v_ub}
\norm{\epsilon_t^b}{2}
\leq \frac{4\sigma_t^2}{\lambda} 
\ \ \text{ and } \ \ 
\Exp_{\z_t}[\norm{\epsilon_t^v}{2}^2  | \calF_{t-1}] \leq 18 \sigma_t^2 \ \ 
\text{ for all } t=1,2,...,N.
\end{equation}
\label{lm:noise_term_control}
\vspace{-0.2cm}
\end{lemma}
\vspace{-0.2cm}
This lemma gives us the dependencies between the variance, bias and clipping level: a larger clipping level leads to a smaller bias but the magnitude of the variance term $\norm{\epsilon_t^v}{2}$ is larger, while the variance of the variance term $\Exp_{\z_t}[\norm{\epsilon_t^v}{2}^2  | \calF_{t-1}]$ remains constant. These three inequalities are also essential for us to use concentration inequalities for martingales. However, we highlight the \emph{necessity} for these inequalities to hold: \emph{the true gradient lies in the clipping region up to a constant}, i.e. $\norm{\nabla \calR(\theta^t)}{2} \leq \lambda / 2$. This condition is necessary since without this, we could not have upper bounds of the bias and variance terms. 
Therefore, the clipping level should be chosen in a very accurate way. Below we informally describe how do we choose it.

We note that $\norm{\theta^t - \theta^*}{2}$ should converge with $1/\sqrt{t}$ rate for strongly convex functions with $O(1/t)$ step size \citep{rakhlin2011making,harvey2019simple}. To make sure  \textit{the first noise term} upper bound by $O(1/i)$ , one should expect each summand  $t\inprod{\epsilon_t^b}{\theta^t-\theta^*} = O(1)$ for $1 \leq t \leq i$, which implies $\norm{\epsilon_t^b}{2} = O(1/\sqrt{t})$.
This motivates us to choose the clipping level to be proportional to $\sqrt{t}$ by Eq.\eqref{eqn:b_and_v_ub}. 
Also, from the detailed proof in Section \ref{sec:proof_clipped_sgd}, we will show that the delay parameter $\gamma$ makes sure $\norm{\nabla \calR(\theta^t)}{2} \leq \lambda / 2$ holds with high probabilities and the position dependent noise $\alpha(P,\loss)$ is controlled.

\paragraph{(iii) Concentration of bounded martingale sequences:} 
A significant technical step of our analysis is the use of the following Freedman's inequality.

\begin{lemma}
\vspace{-0.1cm}
\label{lm:freedman_main_paper}
(Freedman's inequality \citep{freedman1975tail}) Let $d_1, d_2, \cdots,d_T$ be a martingale difference sequence with a uniform bound $b$ on the steps $d_i$. Let $V_s$ denote the sum of conditional variances, i.e. 
$ V_s = \sum_{i=1}^s \var(d_i | d_1,\cdots,d_{i-1}). $
Then, for every $a,v > 0$,
$$
\Pr \left(\sum_{i=1}^s d_i \geq a \ \text{ and } \ V_s \leq v \ \text{ for some }\ s \leq T \right)
\leq \exp \left(\frac{-a^2}{2(v+ba)} \right).
$$
\vspace{-0.4cm}
\end{lemma}
Freedman's inequality says that if we know the boundness and variance of the martingale difference sequence, the summation of them has \emph{exponential concentration} around its expected value for \emph{all subsequence} $\sum_{i=1}^s d_i$.
 
Now we turn our attention to the variance term in \textit{the first noise term}, i.e. $\sum_{t=1}^{i}  (t+\gamma-1) \inprod{\epsilon_t^v  }{\theta^t - \theta^*}  $. It is the summation of a martingale difference sequence since $\Exp[\epsilon_t^v | \calF_{t-1}] = 0$.
Note that Lemma \ref{lm:noise_term_control} has given us upper bounds for boundness/variance for $\epsilon_t^v$.
However, the main technical difficulty is that each summand involves the error of past sequences, i.e. $\norm{\theta^t-\theta^*}{2}$. 

Our solution is the use of Freedman's inequality, which gives us a \emph{loose control} of all past error terms with high probabilities, i.e. $\norm{\theta^t - \theta^*}{2}^2 \leq O\left(N/t^2 \right)$ for $1 \leq t \leq N$. On the contrary, a recurrences technique used in the past works ~\citep{gorbunov2018accelerated,gorbunov2019optimal,gorbunov2020stochastic} uses an increasing clipping levels $\lambda_t$ and calls the Bernstein inequality ( , which only provides an upper bound for the \emph{entire sequence}, ) $N$ times in order to control $\norm{\theta^t - \theta^*}{2}$ for every $t$. As a result, 
it incurs an extra factor $\log(N)$ on their bound since it imposes a too strong control over past error terms.

Finally, we describe why \texttt{clipped-SGD} allows a $O(1)$ batch size at a high level. For previous works of stochastic optimization with strongly convex and smooth objective, they use a constant step size throughout their training process~\citep{gorbunov2018accelerated,prasad2018robust, davis2021low, nazin2019algorithms}. However,  to ensure their approach make a constant progress at each iteration, they should use \emph{an exponential growing batch size} to reduce variance of gradients. Whereas in our approach, we explicitly control the variance by using \emph{a decayed learning rate and clipping the gradients}. Therefore, we are able to provide a careful analysis of the resulted bounded martingale sequences. 

\begin{figure*}[h]
\vspace{-0.4cm}       
\centering
      \subfigure
      %[\label{fig:linear_regression_convergence} \small{Expected convergence curve. }]
      {\includegraphics[width=0.24\textwidth]{figs/linear_regression/gamma_convergence.png} } \hfill
      \subfigure
      %[\label{fig:linear_regression_quantile} \small{Last iteration quantile loss. }]
      {\includegraphics[width=0.24\textwidth]{figs/linear_regression/log_quantile.png}}
      \hfill
      \subfigure
      %[\label{fig:linear_regression_lambda_vs_quantiles}\small{$\log_2(Q_\delta(\theta^N))$ v.s. $\lambda$.}]
      {\includegraphics[width=0.24\textwidth]{figs/linear_regression/lambda_vs_quantile.png}}
      \hfill
      \subfigure
      %[\label{fig:linear_regression_gamma_vs_quantiles}\small{Expected convergence curve for different $\gamma$. }]
      {\includegraphics[width=0.24\textwidth]{figs/linear_regression/convergence_vs_gamma.png} }
\vspace{-0.2cm}    
\caption{Results for robust linear regression for $N=1024, p = 256$, $\gamma=256$ and $\sigma^2 = 0.75$.}
\label{fig:linear_regression}
\vspace{-0.3cm}       
\end{figure*}

